Have I been here before? Learning to Close the Loop with LiDAR Data in Graph-Based SLAM

This work presents an extension of graph-based SLAM methods to exploit the potential of 3D laser scans for loop detection. Every high-dimensional point cloud is replaced by a compact global descriptor, whereby a trained detector decides whether a loop exists. Searching for loops is performed locally in a variable space to consider the odometry drift. Since closing a wrong loop has fatal consequences, an extensive verification is performed before acceptance. The proposed algorithm is implemented as an extension of the widely used state-of-the-art library RTAB-Map, and several experiments show the improvement: During SLAM with a mobile service robot in changing indoor and outdoor campus environments, our approach improves RTAB-Map regarding total number of closed loops. Especially in the presence of significant environmental changes, which typically lead to failure, localization becomes possible by our extension. Experiments with a car in traffic (KITTI benchmark) show the general applicability of our approach. These results are comparable to the state-of-the-art LiDAR method LOAM. The developed ROS package is freely available.

==> kitti_rtabmap_vs_rtabmap+ll.tex <==
\begin{tabular}{l|rrrrrrr}
	%\rule{0pt}{0ex}
	Sequence&00&02&05&06&07&08&09\\
	%Sequence length (m)&3712&5068&2229&1247&695&3231&1722\\
	\hline 
	w/o LL, ATE&1.01&4.4&\textbf{0.51}&0.74&0.48&3.85&2.77\\
	with LL, ATE& \textbf{0.93}&\textbf{4.19}&0.63&\textbf{0.72}&\textbf{0.47}&\textbf{2.9}&\textbf{2.6}\\
	\# visual loops&156&51&88&54&18&0&3\\
	\# LiDAR loops&126&5&72&38&18&30&1\\
	\hline 
	
\end{tabular}

